Integration Error Regularization in Direct Optimal Control using Embedded Runge Kutta Methods

In order to solve continuous-time optimal control problems, direct methods transcribe the infinite-dimensional problem to a nonlinear program (NLP) using numerical integration methods. In cases where the integration error can be manipulated by the chosen control trajectory, the transcription might produce spurious local NLP solutions as a by-product. While often this issue can be addressed by increasing the accuracy of the integration method, this is not always computationally acceptable, e.g., in the case of embedded optimization. Therefore, alternatively, we propose to estimate the integration error using established embedded Runge-Kutta methods and to regularize this estimate in the NLP cost function, using generalized norms. While this regularization is effective at eliminating spurious solutions, it inherently comes with a loss of optimality of valid solutions. The regularization can be tuned to minimize this loss, using a single parameter that can be intuitively interpreted as the maximum allowable estimated local integration error. In a numerical example based on a system with stiff dynamics, we show how this methodology enables the use of a computationally cheap explicit integration method, achieving a speedup of a factor of 3 compared to an otherwise more suitable implicit method, with a loss of optimality of only 3\%.

==> sections/4_example_reaction.tex <==
\section{Example: Catalyst Mixing Problem}

Consider the catalysts mixing problem by \cite{Jaczson1968}, but also discussed by \cite{Biegler2010} and \cite{Bonnans2012}, concerning the reaction of three concentrations of chemicals A,B and C:
\begin{align}
    A \Leftrightarrow B \Rightarrow C
\end{align}
where both reactions are controlled using catalysts, the first reaction is reversible with velocities $k_1, k_2$, and the second reaction has velocity $k_3$.
Using control $u \in [0,1]$ as the fraction of the catalysts and with the state $x(t) = [a(t),\,b(t),\,c(t)]^\top$, the dynamics are then given by:
\begin{align}
    f(x,u) = \begin{bmatrix} \dot{a} \\ \dot{b} \\ \dot{c} \end{bmatrix} = \begin{bmatrix}
        -u(k_1 a - k_2 b) \\ u(k_1 a - k_2 b) - (1 - u)k_3 b \\ (1 - u)k_3 b
    \end{bmatrix}.
\end{align}
It is possible to eliminate the state $c$ due to the invariance $a + b + c = 1$, compare \cite{Jaczson1968,Biegler2010,Bonnans2012}. 
The goal is to maximize the concentration of chemical C at the end of the time interval $t \in [0,t_\mathrm{f}]$, initally the batch consists only of chemical A, i.e. $\bar{x_0} = [1,\,0,\,0]^\top$.
The corresponding OCP is then given by:

\begin{maxi!}
    {x(\cdot), u(\cdot)}{c(t_\mathrm{f})}
    {}{}
    \addConstraint{0}{= x(0) - \bar x_0}
    \addConstraint{\dot x(t)}{= f(x(t), u(t)), \qquad&&\forall t\in [0,t_\mathrm{f}]}
    \addConstraint{0}{\leq u(t) \leq 1, \qquad&&\forall t\in [0,t_\mathrm{f}]} 
  \end{maxi!}
whose optimal solution is, due to \todo{???}, of bang-bang structure, c.f \cite{Biegler2010,Jaczson1968}. 

\paragraph{Discretization} For our example, we consider $k_1 = 50,k_2 = 1, k_3=1, t_\mathrm{f}=1$ and discretize the problem using direct multiple shooting with $N =  20$ integration intervals of length $h  = 1/N$.
Over a single interval, the control is kept constant, the trajectory of $u(t)$ is then parametrized by the $N$ control values $u_0, u_1, \dots u_{N-1}$.
The dynamics are integrated using a explicit Runge-Kutta-Fehlberg method \todo{Butcher Tableau?} of order 5, where for now we only consider the results of the higher order method as a prediction for the state at the end of the interval. 
We would like to point out that for this system, which is very stiff, due to the direct influence of the control $u$ on the dynamics. \todo{Analyze Jacobian e.vs?}, the chosen discretization is not well suited, an implicit integrator should be employed, but for the sake of giving an example, we stick to the unstable explicit integrator.

\todo{Put this somewhere else}
The state trajectory $x(t)$ is then parametrized by the variables $x_i^n, v_i^n$ with subscript index $i = 0, \dots, d$ for the IRK stages and superscript index $n = 0, \dots, N-1$ for the interval. 

The discretized problem is then of the form XX. 


\begin{figure}
    \includegraphics[width=\linewidth]{figures/ChemicalReaction_eps=0.pdf}
    \caption{The solution to NLP XX with $\epsilon = 0$, the large integration error in the first interval falsely maximizes the value of $c(1)$. \todo{Replace plot of $c(t)$ with integration error estimate + true value.}}
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{figures/ChemicalReaction_eps=100.pdf}
    \caption{The solution to NLP XX with $\epsilon = 100$, the optimimum is now a much less aggressive control strategy that is numerically sound.}
\end{figure}

